Regularization can make diffusion models more efficient

Diffusion models are one of the key architectures of generative AI. Their main drawback, however, is the computational costs. This study indicates that the concept of sparsity, well known especially in statistics, can provide a pathway to more efficient diffusion pipelines. Our mathematical guarantees prove that sparsity can reduce the input dimension's influence on the computational complexity to that of a much smaller intrinsic dimension of the data. Our empirical findings confirm that inducing sparsity can indeed lead to better samples at a lower cost.

==> Contents/Furtherdiscussion.tex <==
In the forward process, white Gaussian noise is gradually added to the data with $\x_t=\sqrt{1-\beta_t} \x_{t-1}+\sqrt{\beta_t}\boldsymbol{w}$, where $\boldsymbol{w}\sim \mathcal{N}(\boldsymbol{0},\Identity)$ and  $\beta_t\in (0,1)$ captures the ``amount of noise'' that is injected at time step $t$ and are called the noise schedule. 
\MH{I would just expand $\x_t$ in terms of $\x_{t-2}$ to see how variance looks like then. }
\MH{In general, I think we can just omit the index of the $\boldsymbol{w}$ since they are all Gaussian noise. }
\begin{align*}
 \x_t&=\sqrt{1-\beta_t} \x_{t-1}+\sqrt{\beta_t}\boldsymbol{w} \\
 &=\sqrt{1-\beta_t} \bigl(\sqrt{1-\beta_{t-1}}\x_{t-2}+\sqrt{\beta_{t-1}}\boldsymbol{w}\bigr)+\sqrt{\beta_t}\boldsymbol{w}\\
 &=\sqrt{1-\beta_t} \sqrt{1-\beta_{t-1}}\x_{t-2}+\bigl(\sqrt{(1-\beta_t)\beta_{t-1}}+\sqrt{\beta_t}\bigr)\boldsymbol{w}\,.
\end{align*}
Then, is it true that $\sqrt{(1-\beta_t)\beta_{t-1}}+\sqrt{\beta_t}=\sqrt{1-(1-\beta_t)(1-\beta_{t-1})}$? Seems not! 
But, if we just consider the multiple of the scale of $\x$ that is $\sqrt{\bar{\alpha_t}}$, then we can just say that the variance is its squared complement. 

\begin{equation*}
    \Fd_{t}(\x_t|\x)=\mathcal{N}\bigr(\x_t;\sqrt{\bar\alpha_t}\x,(1-\bar\alpha_t)\Identity\bigl)\,,
\end{equation*}
for $\alpha_t=1-\beta_t$ and $\bar\alpha_t=\prod_{i=1}^{t} \alpha_i$. 

% \subsection{ss}\label{sec:furdisctwo}
% \MH{Here is a note regarding how we compute the objective in (5).  We should find a nice way to adapt it according to our notation $x_t$: Assuming a sequence of $\varnoiseC$ positive noise scales $0<\varnoisemin=\varnoise_1<\varnoise_2<\dots<\varnoise_{\varnoiseC}=\varnoisemax$,
% a scalable alternative for the  objective function in~\eqref{scorematch} is denoising score matching according to~\cite{vincent2011connection} 
% \begin{equation}\label{denoisescorematch}
%  \DnSM\in \arg \min_{\NetP\in \paramspace} \sum_{i=1}^{\varnoiseC}\varnoise_i^2\E_{\disPxCi(\Perx|\x)\p_{0}(\x)}\bigl[\norm{\scoref(\Perx,\varnoise_i)-\nabla_{\Perx}\log \disPxCi(\Perx|\x)}_2^2\bigr]\,, 
% \end{equation}
% where $\Perx$ is a perturbed version of the random vector \x\ based on a pre-specified noise
% distribution $\disPxCi(\Perx|\x)\deq\mathcal{N}(\x,\varnoise_i^2\Identity)$. 

% The marginal distribution of $\Perx$ is $\disPxCi(\Perx)= \int \disPxCi(\Perx|\x) \p_0(\x)d\x$.
%  Note that the estimated neural network $\scorefds(\Perx,\varnoise)$ is a function of two inputs: $\Perx$ and $\varnoise$. 
% As shown in~\cite{vincent2011connection}, the optimization objective  $\E_{\disPxC(\Perx|\x)\p_{0}(\x)}[\norm{\scoref(\Perx,\varnoise)-\nabla_{\Perx}\log \disPxC(\Perx|\x)}_2^2]$ for a fixed variance~$\varnoise$ is equivalent to the optimization  objective $\E_{\disPxC(\Perx)}[\norm{\scoref(\Perx,\varnoise)-\nabla_{\Perx}\log \disPxC(\Perx)}_2^2]$ and, therefore, satisfies $\scorefdssigma(\Perx,\varnoise)=\nabla_{\Perx}\log \disPxC(\Perx)$.
% However, $\scorefdssigma(\x,\varnoise)=\nabla_{\x}\log \disPxC(\x)\approx \nabla_{\x}\log\q_0(\x)$  is true only when the noise is small enough such that $\disPxC(\x)\approx \q_0(\x)$.
% As stated in~\cite{song2019generative}, the denoising score-matching estimator in~\eqref{denoisescorematch} is  consistent once the data distribution lies on a low-dimensional manifold in a high-dimensional ambient space, while other scalable estimators like sliced score-matching~\cite{song2020sliced} are not.
% Therefore, we focus on denoising score matching in this project.
% %as a scalable and consistent alternative for~\eqref{scorematch} in this work. 
% Again, in practice, the expectation in~\eqref{denoisescorematch} needs to be replaced by an average over the training data.
%  We move our attention to a time dependent form of the objective~\eqref{denoisescorematch} in Section~\ref{sec:disc-setting}. }




==> Contents/Intro.tex <==
\section{Starting Point}
\subsection{State of the art and preliminary work}\label{sec:stateoftheart}
\paragraph{State of the art}
Diffusion models have become a popular approach to  probabilistic generative modeling~\parencite{sohl2015deep,song2019generative,ho2020denoising,song2020score,dhariwal2021diffusion,dhariwal2021diffusion,ramesh2022hierarchical}. 
These models progressively destroy  data by injecting noise over time (ending up with pure noise), then learn to reverse this process to generate samples (starting from pure noise) that mimic the distribution of the training data. 
The three predominant formulations of diffusion models consist of denoising diffusion probabilistic models
(\ddpm)~\parencite{ho2020denoising}, score-based generative models (\sgm)~\parencite{song2019generative}, and score-based stochastic differential equations (\sde)~\parencite{song2020score,song2021maximum}.
\ddpm~include two Markov chains: 
a forward process that transforms data into noise, and a reverse process that recovers the data from the noise. 
The objective is to train a function  (usually a deep neural network) for denoising the data over time.
Sample generation then starts with a random Gaussian noise and goes over the trained backward process. 
\sgm~also  perturb data with a sequence of  Gaussian noise and try to estimate the score functions, which is the gradient of the log probability density, for all noisy data. 
For sampling, the trained scores are employed together with score-based sampling approaches like Langevin Monte Carlo~\parencite{grenander1994representations}. 
While~\ddpm\ and~\sgm\ focus on discrete time steps,~\sde~consider infinitely many time steps or unbounded noise levels.
In~\sde, the desired score functions are solutions of stochastic differential equations. 
Once the desired score functions are trained,  sampling can be reached using stochastic or ordinary differential equations.  
Major research on diffusion models concentrates on improving~\ddpm,~\sgm, and~\sde~from three  directions: faster sampling~\parencite{song2020score}, accurate density estimation~\parencite{nichol2021improved},
and handling data with special structures, such as manifolds and manifold structures and discrete data~\parencite{vahdat2021score}. 
This project targets all three directions,  
especially based on~\sgm~(see Section~\ref{sgmintro} for a detailed description of the setting). 

The empirical benefits of diffusion models have been manifested in recent years~\parencite{austin2021structured,dhariwal2021diffusion,rombach2022high}.
The theoretical understanding of these models, on the other hand, is still in its early stages.
The theoretical underpinnings of deep neural networks as the foundation of diffusion models have been explored to some extent~\parencite{Bartlett1998,Anthony2009,Neyshabur2015,Bartlett2017,Hieber2017,kohler2021rate}. 
But these insights have been established in simple frameworks and, therefore, do not apply  to generative models.
The non-asymptotic rates of convergence for diffusion models established very recently~\parencite{block2020generative,de2021diffusion,de2022convergence,lee2022convergence,chen2023probability,chen2023improved,li2023towards,chen2023restoration} show the large interest in this topic and are an important step forward but do not fully explain the success of generative models either.
For example, results like~\textcite[Theorem~13]{block2020generative} provide rates of convergence for diffusion models in terms of Wasserstein distance, 
but they suffer from the curse of dimensionality in that the rates depend exponentially on the dimensions of the data, that is, the number of input features. 
\textcite{block2020generative} 
 study convergence of Denoising Auto-Encoders (DAE) and Denoising Score Matching (DSM) using Langevin diffusion for sampling by employing the tools from empirical-process theory.
 %~\parencite{Sara2000,Vershynin2018}.
 %They also show that DAE and DSM objectives are equivalent up to an affine transformation~\parencite[Proposition~5]{block2020generative}.
 Recent works then concentrate on improving convergence guarantees to grow polynomially in the number of input features under different assumptions on the  original and estimated scores ($L_2$-accurate score estimates, Lipschitz or smooth scores, scores with bounded moments)~\parencite{lee2022convergence,chen2022sampling,wibisono2022convergence,chen2023probability,chen2023improved,chen2023restoration,lee2023convergence}. 
 For example,~\textcite {lee2022convergence} prove a convergence guarantee  in terms of total variation for~\sgm, 
 which has a polynomial dependence on the number of input features if the score estimate is $L_2$-accurate for any smooth distribution satisfying the log-Sobelev inequality.
 %Their rates grow polynomially in the dimension of the data under some additional assumptions. 
A very recent work by~\textcite{li2023towards} proposes improved convergence rates in terms of total variation for~\ddpm~with ordinary differential equations and stochastic differential equations samplers that are proportional to $\Dim^2/\error$ under mild assumptions,
where $\Dim$ is the number of input features and $\error$ the error in the measure under consideration.
Formulated differently, to achieve $\tv(\p_0,\q_0)\le \error$ (meaning that the total variation between the estimated distribution $\q_0$ and the true distribution $\p_0$ is not larger than $\error$), the number of diffusion steps $\T$ needs to grow by $O(\Dim^2/\error)$.\footnote{For two density functions~$\p$~and~$\q$ on $\mathcal{X}$~with respect to a base measure~$\nu$, we define $\tv(\p,\q)\deq\frac{1}{2}\int_{\mathcal{X}}|\p(\x)-\q(\x)|\nu(d\x)$~\parencite{wainwright2019high}.} 
This can be very challenging when dealing with high-dimensional data, that is, when $\Dim$ is large.
\textcite[Theorem~3]{li2023towards} also provides rates that grow by~$O(\Dim^3/\sqrt{\error})$ for an accelerated ordinary differential equations samplers. 
While works like~\textcite{li2023towards} concentrate more on improving the rates in~$\error$,~\textcite{chen2023probability} focus on improving the rates in~$\Dim$. 
\textcite{chen2023probability} use a specially chosen corrector step based on the underdamped Langevin diffusion to achieve their improvements (namely $O(\sqrt{\Dim}/\error)$ vs.~$O(\Dim/\error)$) 
by assuming: 1.~the score function along the forward process is $L$-Lipschitz,  2.~the data distribution has a finite second moment, and  3.~there is access to accurate scores. 

To summarize,
the discussed papers are important advances in the field,
but the  polynomial dependence of the rates on $\Dim$ is a major open problem.
For example, in text and image generation, $\Dim$ can easily be of the order of millions,
while empirical studies show that diffusion models are still performing very well in these settings.
Thus, there is still a large gap between theory and practice of diffusion models.

%of diffusion models and the question of whether these rates can be improved, more specifically in terms of the factor $\Dim$), further or not.


\paragraph{Other related work} 
Other theory-related papers for diffusion models target the convergence  rates and robustness of diffusion models~\parencite{pidstrigach2022score}, approximation and generalization capabilities of diffusion modeling for distribution estimation~\parencite{oko2023diffusion}, and study the information behind the approximated score functions~\parencite{batzolis2022your} that are still close to our study here. 
Also, recently,~\textcite{montanari2023posterior} and~\textcite{el2022sampling} have studied sampling from posterior distributions using the idea of stochastic localization. 
The statistical efficiency of score matching has been also investigated by~\textcite{koehler2022statistical}.
But none of these papers fill the above-mentioned gap in the literature.





\paragraph{Preliminary work}
The PI has done extensive research on the pillars of this project, 
namely 
% ~\parencite{BoTh12} \parencite{lederer2022fundamentals,Buhlmann11}
generative modeling and scores~\parencite{laszkiewicz2021copula,laszkiewicz2022marginal,lederer2023extremes},
regularization~\parencite{lederer2022fundamentals,Hebiri13, Gold17,hebiri2020layer,taheri2021},
and concentration  inequalities~\parencite{Lederer13b,Lederer2014}. 
The project also draws on the PI's extensive expertise in tuning-parameter calibration~\parencite{Bunea14,chichignoud2016practical,chetelat2017optimal,laszkiewicz2021thresholded,LedererVogt20,huang2021tuning,lederer2022topology,taheri2022balancing}
and the intricacies and inaccuracies of convex and non-convex optimization~\parencite{bien2018non, lederer2020optimization,taheri2022balancing,taheri2022statistical}.







% \paragraph{Long-term vision of the project}
% In the long-term vision, this project aims to improve the performance of baseline diffusion models in terms of accuracy and computational time. 
% That is, we would improve the application of diffusion models for huge-real datasets. 
% So, we not only consider theory but also the application of proposed methods in real-world problems. 
% In future research, we plan to use our results in biology (with our collaborator Dr.~Li-Xuan Qin, Sloan Kettering) and medicine (with our collaborator Dr.~Kristoffer Hellton, Norwegian Computing Center)---and we believe that many other researchers might use our results in their fields as well.




% \subsection{Project-related publications}
% \subsubsection{Articles published by outlets with scientific quality assurance, book publications, and works accepted for publication but not yet published}
% \begin{enumerate}[]
%    \item \fullcite{lederer2022fundamentals}
%    \item \fullcite{chichignoud2016practical}
%    \item \fullcite{taheri2022balancing}
% \item \fullcite{taheri2021}   
% \item \fullcite{YoyoSara12}
% \item \fullcite{laszkiewicz2022marginal}
% \item \fullcite{bien2018non}
% \end{enumerate}


% The first three papers illustrate the PI’s expertise in sparsity and high-dimensional prediction and inaccuracy in the computation of sparse estimators.
% The other paper illustrates the PI’s expertise in the theory of sparse neural networks. 
% The last three papers illustrate the PI’s expertise in empirical process theory, generative modeling, and non-convex optimization.
% These concepts are the basis of this project.
% \subsubsection{Other publications
% }
% \begin{enumerate}[]  
% \item \fullcite{lederer2023extremes}
% \item \fullcite{laszkiewicz2021copula}
% \item \fullcite{taheri2022statistical}
% \item \fullcite{lederer2020optimization}


% \end{enumerate}
% The first two papers illustrate the PI’s expertise in generative modeling. 
% The other papers illustrate the PI’s expertise in the theory of deep neural networks, approximate estimators, and non-convex objectives. 
% The papers are currently under review for top-tier outlets.





\paragraph{Contributions of this project}

This project will make three main contributions:
\begin{itemize}
    \item 
    \textbf{WP1:}
    We develop an approach for estimating an unknown distribution $\p_0$, having in mind that this estimate will be used to generate approximate samples from $\p_0$. 
    Assume that the  target distribution $\p_0$ lies on a low-dimensional manifold of dimension $\sm$ in a high-dimensional ambient space of dimension $\Dim$, $\sm\ll \Dim$,
    we will improve the rates of convergence from $O(\Dim^2/\error)$ to essentially $O(\sm^2/\error)$.
    
%We  propose an approach to accelerate the sampling process of diffusion models using denoising score-matching estimator. 
%The main idea of this section is to employ the valuable information behind the estimated score function to lead the sampling process more efficiently. 
%We will show that by employing the proposed method together with an appropriate sampler, the sampling process of diffusion models can speed up from $O(\Dim^2/\error)$  to $O(\sm^2/\error)$. 
%We will also apply the proposed method on simulated data. 
\item 
\textbf{WP2:}
We then develop an approach that allows for more general setups,
no longer assuming that the unknown distribution lies on a low-dimensional manifold.
We will use regularization and show that the rates can still be improved from $O(\Dim^2/\error)$  to essentially $O(\EfDim^2/\error)$, where again $\EfDim\ll \Dim$,
if the true score function can be approximated by a sparse neural network.
We also establish a provably accurate scheme for calibrating the corresponding tuning parameter.
%
%Furthermore, we improve rates of convergence of diffusion models for general target distribution   employing the tools from high dimensional statistics. 
%We propose a regularized objective for score-matching, motivated to push some prior information for the desired score function. 
%We will show that by employing a suitable penalty function, together with a large enough tuning parameter, the rates of convergence for diffusion models can be improved from $O(\Dim^2/\error)$  to $O(\EfDim^2/\error)$, with $\EfDim\ll \Dim$.
%We also propose employing an adaptive validation approach for tuning parameter calibration that considerably improves the computation time in comparison with other approaches like cross-validation. 
%We will validate the proposed method on simulated data. 
\item 
\textbf{WP3:}
We finally connect those statistical methods and theories with aspects from optimization by considering approximate rather than exact computations of the minimizers of the score-based objectives.

%Finally, we move toward considering the optimization difficulties of non-convex objectives  for diffusion models. 
%We develop convergence rates for approximation of regularized score matching and regularized denoising score matching that are close to the global minimizer and not exactly equal to it. 
%We will show that even estimators in a close neighborhood of the global minimizers can still generalize well in the context of diffusion models. 
%We also validate our proposed theory on simulated data. 
\end{itemize}
